A Lower Bounding Framework for Motion Planning amid Dynamic Obstacles in 2D

This work considers a Motion Planning Problem with Dynamic Obstacles (MPDO) in 2D that requires finding a minimum-arrival-time collision-free trajectory for a point robot between its start and goal locations amid dynamic obstacles moving along known trajectories. Existing methods, such as continuous Dijkstra paradigm, can find an optimal solution by restricting the shape of the obstacles or the motion of the robot, while this work makes no such assumptions. Other methods, such as search-based planners and sampling-based approaches can compute a feasible solution to this problem but do not provide approximation bounds. Since finding the optimum is challenging for MPDO, this paper develops a framework that can provide tight lower bounds to the optimum. These bounds act as proxies for the optimum which can then be used to bound the deviation of a feasible solution from the optimum. To accomplish this, we develop a framework that consists of (i) a bi-level discretization approach that converts the MPDO to a relaxed path planning problem, and (ii) an algorithm that can solve the relaxed problem to obtain lower bounds. We also present numerical results to corroborate the performance of the proposed framework. These results show that the bounds obtained by our approach for some instances are up to twice tighter than a baseline approach showcasing potential advantages of the proposed approach.

==> related.tex <==

% \noindent\textbf{Motion planning}~\cite{choset2005principles,lavalle2006planning} is a fundamental robotics problem and has been widely studied.
% In the presence of dynamic obstacles, various methods have been developed to compute optimal or near-optimal solutions:
% To name a few, search-based algorithms~\cite{phillips2011sipp,yakovlev2021towards} discretize the workspace into a graph and run A*-like heuristic search to find an optimal solution with respect to the graph, whose quality is determined by the underlying graph discretization.
% Sampling-based methods~\cite{lavalle2006planning,hsu2002randomized} iteratively sample and evaluate points from the workspace to compute asymptotic-optimal trajectories with infinite samples~\cite{lavalle2006planning} or near-optimal trajectories with finite samples~\cite{dayan2021near}.
% Continuous Dijkstra~\cite{fujimura1994motion,hershberger1999optimal} as well as its recent variants~\cite{maheshwari2020shortest} typically put restriction on the shape of the obstacles (e.g. polygonal obstacles) and then find optimal trajectories.
% This type of algorithms has not yet been thoroughly evaluated numerically.
% Path-velocity decomposition methods~\cite{kant1986toward} first find a path and then plan the velocity along the path to avoid obstacles.
% All these methods can compute a feasible ($i.e.$ collision-free) trajectory for the motion planning problem considered in this work, whose cost is an upper bound of $C^*$.
% This work differs from them as the focus here is to compute tight lower bounds of $C^*$.

% \vspace{1.5mm}
% \noindent\textbf{Computing lower bounds} for planning problems arises in many applications.
{\color{blue} Not sure if this related work section is still needed. But I am afraid "computing lower bound" will remind people about the following related works. In addition, should we mention the DTSP work?} 

Computing lower bounds for motion planning arises in many applications.
For instance, in high-dimensional motion planning problems~\cite{cohen2014single}, the original problem is often relaxed to a low-dimension problem to fast compute lower bounds, which are then used as heuristic values to better guide the full-dimensional planning.
In multi-agent path finding problems~\cite{sharon2015conflict}, the potential collisions between agents are often ignored at first to compute individual optimal paths, which are then used to guide the subsequent multi-agent search.
These methods aim to fast compute lower bounds ($i.e.$ heuristic-values) that can effectively guide the planning, and the tightness of the bound is not the primary goal.
This work differs from them as our goal is to compute tight lower bounds.

Tight lower bounds can provide optimality estimation to justify how far a feasible solution is away from being optimal.
%The challenge is to recognize the aspect of the original problem that can be relaxed, and formulate a lower bounding problem to provide tight lower bounds.
As an example, in dubins traveling salesman problems~\cite{manyam2018tightly}, given a feasible solution, the optimality estimation computed by using a naive lower bound can be significantly looser than using a tight lower bound~\cite{manyam2018tightly}.
In this work, our numerical results show that the lower bounds computed by our approach can lead to much tighter optimality certificates for a feasible solution than naively using Euclidean distance as the lower bound.

% \noindent\textbf{Contributions} of this work are:
